Not one but many Tradeoffs: Privacy Vs. Utility in Differentially Private Machine Learning

Data holders are increasingly seeking to protect their user's privacy, whilst still maximizing their ability to produce machine models with high quality predictions. In this work, we empirically evaluate various implementations of differential privacy (DP), and measure their ability to fend off real-world privacy attacks, in addition to measuring their core goal of providing accurate classifications. We establish an evaluation framework to ensure each of these implementations are fairly evaluated. Our selection of DP implementations add DP noise at different positions within the framework, either at the point of data collection/release, during updates while training of the model, or after training by perturbing learned model parameters. We evaluate each implementation across a range of privacy budgets, and datasets, each implementation providing the same mathematical privacy guarantees. By measuring the models' resistance to real world attacks of membership and attribute inference, and their classification accuracy. we determine which implementations provide the most desirable tradeoff between privacy and utility. We found that the number of classes of a given dataset is unlikely to influence where the privacy and utility tradeoff occurs. Additionally, in the scenario that high privacy constraints are required, perturbing input training data does not trade off as much utility, as compared to noise added later in the ML process.

==> sections/framework.tex <==
% !TEX root =  ../ccs2020.tex
%-------------------------------------------------------------------------------
\section{\DP-enabled ML FRAMEWORK}\label{sec:framework}
%-------------------------------------------------------------------------------
The framework is quite straightforward, with any given dataset, it is passed through the \DP-enabled ML framework, once the model is produced, a utility metric, and/or privacy metric is evaluated. 

In our work we focus on an instantiation of this framework to evaluate the tradeoff between privacy (as measured through MI and AI attacks) and utility (as measured by Accuracy Loss) in privacy-preserving machine learning algorithms.
In particular, we present and explain the ML framework used, in which we introduce \DP noise in three Stages of the learning process.
In addition, we present algorithmic formulations for the four ML methods explored in the study, using the \DP noise applied at the different stages.


\subsection{\DP-enabled ML Framework}

\begin{figure*}[t]
	\centering
	\includegraphics[width=0.90\textwidth]{figs/eval_pipeline_new.pdf}
	\vspace{-4mm}
	\caption{The proposed ML framework with the possible Stages that \DP noise can be introduced to guarantee privacy.}
	\label{fig:eval_pipe}
\end{figure*}

As noted by~\cite{jayaraman2019evaluating}, there are three general positions in which \DP noise can be applied to a ML task, to preserve privacy of the data used, or the model built.
These three positions of entry in the ML framework are visualized in Figure~\ref{fig:eval_pipe}.
To make the next observations more concrete, let the function $\mathcal{F}$ map the training dataset \textbf{X} to class labels \textbf{y}, that is, $\mathcal{F}(\textbf{X}) = \textbf{y}$.
Then, the goal of the ML model is to approximately learn this relationship between dataset and labels as best as possible.

Next, we discuss each of these three framework Stages:


\noindent
\textbf{\textit{Stage 1 (S1):}} \textit{During the collection or release of data.}
During data (\textbf{X}) production or collection, and before aggregation at the server, if local \DP noise is applied on every data record, the records (\textbf{X'}) can be protected before being used in a ML framework.
Alternatively, when releasing a dataset to the public domain, the owner can train a data generator to create a synthetic dataset containing the same data semantics as the real data, but with the synthetic data governed by the rules of \DP.
Next, the $\mathcal{F}$(\textbf{X'}) model learned is \DP-enabled.

\noindent
\textbf{\textit{Stage 2 (S2):}} \textit{During the learning process.}
In this stage, each step of the model update is restricted as to not excessively alter the model with the added \DP noise ($\mathcal{F'}$(\textbf{X})), and thus compromise the privacy of a given batch of records.
The classic example for this Stage is the Tensorflow Privacy, which deploys a \DP stochastic gradient descent algorithm~\cite{abadi2016deep}.

\noindent
\textbf{\textit{Stage 3 (S3):}} \textit{After the learning process.}
After the data modeling has finished, the learned parameters of the model can be perturbed, by adding \DP noise on them ($\mathcal{F'}$(\textbf{X})) to remove dependencies between learned parameters and training data.


We remark that in contrast to~\cite{jayaraman2019evaluating} which focuses primarily on DP compositions for S2: Neural networks, and S3: Logistic Regression, they do not offer a direct comparison with respect to the machine learning algorithm itself, only that they both leverage empirical risk minimization in the learning process. In this work, we explore various \DP-based ML methods that are applicable in each of these Stages outlined.


\subsection{\DP-based ML Algorithms}
\label{sec:algorithms}

After reviewing the literature on existing ML methods that have been modified to provide \DP protection to the data or model, we have identified various such realizations that can be divided in the three Stages outlined above.
In this work, we identified four key ML algorithms for classification that are of interest: Naive Bayes (\NB), Logistic Regression (\LR), Random Forests (\RF), and Neural Networks (\NN).
Next, we describe the approach used by each of these algorithms in learning on data in a supervised setting, while applying \DP noise in the ML framework, in each of the Stages identified earlier.
In Table~\ref{tab:exec_dp_ways} we summarize the ML methods used per Stage.

\begin{table}[ht]
\vspace{-1mm}
\caption{\DP-based ML methods used in the \DP-enabled ML framework Stages.}
\label{tab:exec_dp_ways}
\vspace{-3mm}
\centering
\resizebox{0.7\columnwidth}{!}{%
\begin{tabular}{p{3cm}p{1.0cm}p{1.0cm}p{0.8cm}}
\toprule
				 \multicolumn{4}{r}{Stage where \DP noise is applied}	\\
ML Method		&	S1	&	S2	&	S3			\\
\midrule
\rowcolor[HTML]{EFEFEF}
Naive Bayes		&	X	&		&	X			\\
Logistic Regression	&	X	&		&	X			\\
\rowcolor[HTML]{EFEFEF}
Random Forests	&	X	&	X	&				\\
Neural Network		&	X	&	X	&				\\
\bottomrule
\end{tabular}
}
\vspace{-2mm}
\end{table}


\subsubsection{S1: Manipulation of Laplacian Noise}

At this Stage, we apply \DP Laplacian noise~\cite{das2016tracking} directly on the dataset, and thus, this process is independent of the ML algorithm used in subsequent steps of the framework.
As a result of this independence, we can employ all four ML algorithms, in their non-private versions, and use them on the modified, \DP data.
In particular, \DP is provided by the addition of noise to every vector in the dataset.
Laplacian noise is independently sampled for every feature value, of every data vector from the distribution $Lap(0, \beta_i)$, where $\beta_i = \frac{S_i}{\epsilon/p}$, and $S_i$ is the value range of the $i$th feature~\cite{das2016tracking} (Algorithm~\ref{alg:dp-data}).

\begin{algorithm}[ht]
	\SetAlgoLined
	\KwIn{Training Dataset \textbf{$X$}, where $x := \{x_0, ..., x_i, ...,x_p\}$}
	\KwResult{Differentially private Training Dataset \textbf{$X'$}}

	\For{$x$ in $X$}{
		$x' = x + b;$ 
		where $b:= \{b_0, ..., b_i, ...,b_p\}; b_i \in Lap(0, \beta_i)$
	}

	Proceed with learning task $\mathcal{F}$ on \textbf{$X'$}.
\vspace{1mm}
\caption{Direct addition of \DP noise to dataset before use by ML framework.}
\label{alg:dp-data}
\end{algorithm}


Adding \DP noise in this Stage is ML independent and permits more flexibility, as any ML or DL method can be employed after this Stage for training.
The application of noise is dependent on the data types and their complexity with respect to features and values allowed. 

\begin{remark}
\DP noise is applied with the assumption that features are independent from each other, meaning a maximal amount of noise must be applied to each feature to ensure \DP. With knowledge of feature dependence, hypothetically less noise can be applied to the dependent features as there is less uniquely identifying information between the dependent features.
\end{remark}

\subsubsection{S2: \DP-based Random Forests}

Random Forests (\RF)~\cite{NIPS2012_4824} are an ensemble of decision trees produced through bagging (bootstrap aggregation), whereby the training dataset is resampled from the training data to introduce dataset variability in the training of each tree.
By applying feature randomization, a restriction in the number of features available to a tree when splitting a leaf node, the \RF is able to produce an ensemble of varied trees each with its own decision, from which the final classification decision is made (for example majority vote).
Differentially private random forests with Smooth Sensitivity~\cite{fletcher2017differentially} create conventional random forests, but instead of retaining the exact frequencies of data under each subsequent branch from the leaf, only the majority label is retained after the application of an exponential mechanism dependent on the privacy budget available (Algorithm~\ref{alg:dp-rf}):


\begin{algorithm}[ht]
	\SetAlgoLined
	\KwIn{Boosted and Bagged Training Dataset \textbf{$X$}}
	\KwResult{Differentially private decision tree \textbf{$T'$}}
	Compute $T$, a regular tree from $X$;

	\For{each node within the tree}{
		retain \texttt{Majority Label} from datapoint frequencies through exponential mechanism~\cite{fletcher2017differentially};
	}
	Return \textbf{$T'$} to the Forest;
\vspace{1mm}
\caption{\DP-based \RF with Smooth Sensitivity~\cite{fletcher2017differentially}.}
\label{alg:dp-rf}
\end{algorithm}



\begin{remark}
Computing the confidence of a prediction from the \RF has been complicated due to the omission of distributions in the leaf nodes of trees.
It is however possible for us to compute a confidence value from the majority voting aggregation of predictions of trees within the random forest.
\end{remark}

\subsubsection{S2: \DP-based Neural Networks}

Neural Networks (\NN) are designed to mimic the functionality observed within brains~\cite{gurney2014introduction}.
They contain multiple layers of neurons (some hidden) that are activated depending on the activation of neurons in the previous layer. 
The influence of a previous layers' neurons on the current neuron varies depending on a weight or parameter value learned during the training phase.
The very final layer is often a decision layer that corresponds to each of the classes present in the classification problem.
The degree of activation of this last layer is analogous to the \textit{confidence} of the class prediction.

The approach employed by Tensorflow-Privacy's~\cite{abadi2016deep} implementation of \DP-enabled \NN involves the use of a \DP stochastic gradient decent (SGD) algorithm.
The SGD algorithm seeks to find network parameters $\theta$ to learn function $\mathcal{F}$.
The \DP-based SGD first clips or limits the size of the gradient update, so that it is not heavily impacted by one batch of data.
Additional noise is added to the updated gradient depending on the values of $\epsilon$, and batch sensitivity (Algorithm~\ref{alg:dp-nn}):

\begin{algorithm}[ht]
	\SetAlgoLined
	\KwIn{Training Dataset \textbf{$X$}}
	\KwResult{Differentially private parameters $\theta'$ }

	$\theta' \leftarrow \texttt{RAND}$, initialize the parameters randomly;

	\For{batch $t \in T$}{
		%Compute Gradients
		compute gradient $\Delta \theta$,
		clip gradients $\Delta \theta$,
		add DP-noise $b$
		
		$\theta' = \theta' + \Delta\theta + b$
	}
	Complete $\mathcal{F}'$ learning task with $\theta'$.
\vspace{1mm}
\caption{\DP-based Stochastic Gradient Decent~\cite{abadi2016deep}.}
\label{alg:dp-nn}
\end{algorithm}



\subsubsection{S3: \DP-based Naive Bayes}

The Naive Bayes (\NB)~\cite{rish2001empirical} classification algorithm learns probabilistic distributions of the output classes informed by the input feature values.
The algorithm is considered ``naive'', as it assumes an independence between features.
The distributions are learned directly from the training dataset.
The simple formulation of the model enables the Naive Bayes classifiers to both be trained, and to make predictions relatively quickly.

IBM Naive Bayes~\cite{holohan2019diffprivlib} implements an $(\epsilon)$-\DP Naive Bayes, originally proposed by~\cite{vaidya2013differentially}.
The approach adds noise to the learned distributions that relate the input feature to the output decision.
Algorithm~\ref{alg:dp-nb} shows the addition of Laplacian noise to the mean and standard deviation ($\mu$, $\sigma$) computed from training dataset $X$.
A more complete algorithm for handling both categorical and continuous data can be found in~\cite{vaidya2013differentially}.

\begin{algorithm}[ht]
	\SetAlgoLined
	\KwIn{Training Dataset \textbf{$X$}}
	\KwResult{Differentially private model distributions \textbf{$\theta'$}}
	Compute (\textbf{$\mu$, \textbf{$\sigma$}}) from \textbf{$X$};
    
	\For{$i$ in $features$}{
		Compute scaling factor $S_{(\mu,i)}$ and $S_{(\sigma,i)}$ from feature mean $\mu_i$, feature STD $\sigma_i$, and $\epsilon$;

		$\mu_i' = \mu_i + b_i$;
		where $b_i \in Lap(0, S_{(\mu,i)})$;
    
		$\sigma_i' = \sigma_i + b_i$;
		where $b_i \in Lap(0, S_{(\sigma,i)})$;
	}
	Compute output priors $P(y|x)$ from (\textbf{$\mu'$, \textbf{$\sigma'$}});
\vspace{1mm}
\caption{\DP-based Naive Bayes provided by IBM~\cite{holohan2019diffprivlib}.}
\label{alg:dp-nb}
\end{algorithm}



\subsubsection{S3: \DP-based Logistic Regression}

The Logistic Regression (\LR)~\cite{mccullagh2019generalized} algorithm employs the logistic function (sigmoid function) to model the probability of a binary outcome (binary classification) in relation to the input feature vector.
In the multi-class setting, every output class has an independent logistic function predicting the binary objective of the specific class (or not).
The final classification is an aggregation of these independent functions.

\DP-based Logistic Regression~\cite{chaudhuri2011differentially} works by adding Laplacian noise proportional to the Sensitivity of the feature and $\epsilon$ to the objective function of the model (loss function).
After the noise addition, $\mathcal{F}'$ can be evaluated (Algorithm~\ref{alg:dp-lr}):

\begin{algorithm}[th]
	\SetAlgoLined
	\KwIn{Training Dataset \textbf{$X$}}
	\KwResult{Differentially private objective function $\mathcal{J}'$}
	Compute (\textbf{$\mu$, \textbf{$\sigma$}}) from \textbf{$X$};

	$\mathcal{J}' = \mathcal{J} + \textbf{b}$;

	where $\textbf{b} \in Lap(0, \beta)$; specific details on $\beta$ available in \cite{holohan2019diffprivlib}

\vspace{1mm}
\caption{\DP-based Logistic Regression by IBM~\cite{holohan2019diffprivlib}.}
\label{alg:dp-lr}
\end{algorithm}

\begin{remark}
We regard the minimization of the objective function on the noisy objective function of \LR as Stage 3, as the \DP noise is applied with access to the entire set of data, and the noise is not dependent on any partial split of the data.
\end{remark}

